Through the Looking-Glass: Transparency Implications and Challenges in Enterprise AI Knowledge Systems

Knowledge can't be disentangled from people. As AI knowledge systems mine vast volumes of work-related data, the knowledge that's being extracted and surfaced is intrinsically linked to the people who create and use it. When predictive algorithms that learn from data are used to link knowledge and people, inaccuracies in knowledge extraction and surfacing can lead to disproportionate harms, influencing how individuals see each other and how they see themselves at work. In this paper, we present a reflective analysis of transparency requirements and impacts in this type of systems. We conduct a multidisciplinary literature review to understand the impacts of transparency in workplace settings, introducing the looking-glass metaphor to conceptualize AI knowledge systems as systems that reflect and distort, expanding our view on transparency requirements, implications and challenges. We formulate transparency as a key mediator in shaping different ways of seeing, including seeing into the system, which unveils its capabilities, limitations and behavior, and seeing through the system, which shapes workers' perceptions of their own contributions and others within the organization. Recognizing the sociotechnical nature of these systems, we identify three transparency dimensions necessary to realize the value of AI knowledge systems, namely system transparency, procedural transparency and transparency of outcomes. We discuss key challenges hindering the implementation of these forms of transparency, bringing to light the wider sociotechnical gap and highlighting directions for future Computer-supported Cooperative Work (CSCW) research.

==> faithfulness_versions.tex <==
\item \textbf{Faithfulness and access:} One way to make transparent how AI knowledge systems extract knowledge associations from work-related data involves making visible the pieces of work being mined by the system. This data might be created by different individuals belonging to different teams and sub-organizations, and since many organizations have file access rules and privacy settings that vary depending on membership of departments and teams, people's access to sources of information may vary from person to person.
    % For example, depending on the organization, access controls might prevent individuals from accessing documents authored by others in a different team or in a different geographical location. These rules and controls might be in place to help prevent information being leaked outwards, such as product development documentation not being accessible to customer-facing teams.
    In practice, this means that while an AI knowledge system might use different pieces of work to relate people to knowledge, these pieces of work (sometimes referred to as ``evidence'') may not be accessible to the end-users who see the surfaced associations. This can have different implications for how individuals see \emph{into} the system, as well as how they see others in their organization \emph{through} the system and how they see themselves. 
    
    To illustrate the impacts when seeing \emph{into} the system, in global organizations legal requirements and restrictions might prevent data transfer across geopolitical boundaries, leading to different configurations of access controls. These constraints might prevent people from seeing knowledge contributions or documents authored by people in a different location. If knowledge contributions are used to explain system associations, this would lead to inconsistent explanations across end-users: While those who can access the documents would be in a better position to understand system behavior, this is not the case for those who can't see the documents supporting the associations.% might not understand, and decide not to act upon, the inferences made by the system. 
    
    When different people have access to different knowledge contributions and resources, different ways of seeing others in the organization may also affect interpersonal aspects such as perception of competence, potentially leading to allocative harms via second order effects. As an example, if the system shows that both Liza and David work on a given knowledge area, the documents and knowledge resources Liza and David contributed to may be used by other users to make inferences about their relationships with that knowledge area. % could be used as a way to explain the provenance of the surfaced information.
    If a given individual can access five documents authored by Liza and only one authored by David, they might (consciously or not) assume that Liza has greater expertise than David. If this is a pattern across multiple users, this could over time skew the relative amount of visibility and exposure Liza and David get, in effect erasing David's labor.
    % the system might induce greater perception of expertise on Liza, making Liza's work visible while limiting the exposure and potentially erasing David's labor.
    % When using work contributions as a mechanism for system transparency,
    Other access constraints on the source data such as language barriers can similarly lead to allocative harms that limit individuals' opportunities for recognition. For instance,% in a global organization, different contributors might create and work on documents in different languages. If sources aren't translated or if the translation leads to different levels of quality, leaders in the organization might see members in different locations differently. For example, a director based in an English-speaking country might be able to read the documents supporting the associations of English-speaking individuals, while not be able to understand the original pieces of work supporting the associations of team members in non-English speaking countries such as Japan or France.
    if different contributors create and work on documents in different languages, and sources aren't translated or translation leads to different levels of quality, leaders in the organization might see members in different locations differently, most likely to the detriment of employees with a different working language than the leadership.

    Finally, using work-related data as a way to explain system behavior also raises challenges when providing transparency to users about their own associations to knowledge. In principle, the resources used to make inferences about an individual can include resources that they do not have access to, such as human resources documents or other people's emails and chats that mention the individual. The inability to expose these pieces of data prevents the individual from getting the full picture of why they're represented in the system in the way they are. As an example, we may imagine that an individual finds that they've been associated to a topic they haven't worked on.
    % Let us imagine that the association is inferred using document sources authored by leadership teams, detailing a future readjustment and reallocation of resources in the company. By drawing on this data, the association itself is leaking sensitive information that hasn't been communicated to employees yet. As the individual tries to work out an explanation for the association, they may start imagining these kinds of connections, with potential negative personal or organizational impact.
    Imagine that the association has been inferred from, among other things, personal chat communication between the individual's team members as they coordinate work. Informing the individual that some of the evidence for the association can’t be exposed due to privacy constraints can have a deep impact on the beliefs that individual holds about how they’re being seen by others in the organization: Is their continued employment being discussed in emails among management? Has someone made a complaint about them that has been documented in a human resources file? This impact on meta-perceptions, or imagined attitudes and opinions of others, can influence self-efficacy beliefs and self-esteem, directly affecting their behavior and interpersonal relationships within the organization. As this example shows, knowledge access systems that automatically extract and surface knowledge relationships from work-related data integrate and enforce a layer of transparency in the social context of the organization, directly or indirectly exposing information that people might have chosen not to bring attention to. Furthermore, failing to be transparent about how these associations have been formed can negatively affect the productivity and well-being of employees, as it hinders their ability to understand and assess the validity of system outputs and limits their agency to exercise control over how they are represented at work.

    These two examples show that not only can discrepant access to organizational data result in an incomplete picture of the system, but negative consequences can follow both from incorrect assumptions of completeness and from attempts to fill in the gaps of the incompleteness.
    % LONGER VERSION: These two examples show that not only can discrepant access to organizational data result in an incomplete picture of the system, but negative consequences can follow both from incorrect assumptions of completeness and from attempts to fill in the gaps of the incompleteness, as they shape how people see \emph{into} the system and \emph{through} the system. As the examples demonstrate, such partial transparency can lead to interpersonal, representational and quality of service harms. Moreover, given that organizational privacy rules and access constraints may enforce existing power dynamics and asymmetries, partial transparency can further exacerbate that.
    
    % all documents in an organization are potential sources of expertise evidence since they are created by or about somebody \cite{yimam2003expert}. This means that sources that aren't accessible to a given individual can be used to relate that individual to a given area of work. These sources might include private unstructured data, such as emails or chats, or highly sensitive documents such as human resources data. The inability to expose these pieces of data prevents an individual to understand why they're represented in the system in a certain manner and appropriately interpret the algorithmic reflections of their work. As an example, we consider the case of an individual being associated to a topic they haven’t worked on and not understanding where the association comes from. Let us imagine that the association is inferred using document sources authored by leadership teams, detailing a future readjustment and reallocation of resources in the company. The association itself is leaking sensitive information that hasn't been communicated yet, potentially impacting the individual, who might start imagining different reasons in an attempt to explain the association themselves. Another example might involve mining knowledge associations using private source data such as chats. Communicating to an individual that the sources influencing the association can’t be exposed due to privacy constraints can have a deep impact on the beliefs an individual holds about how they’re being seen by others in the organization. This impact on meta-perceptions, or imagined attitudes and opinions of others, can influence self-efficacy beliefs and individual self-esteem, directly affecting their behavior and interpersonal relationships within the organization. By automatically extracting and surfacing knowledge relationships from work-related data, AI-mediated knowledge access systems already integrate and enforce a layer of transparency within the social context of the organization, exposing information that people might have chosen to keep hidden. Failing to be transparent into how these associations have been formed can negatively affect the productivity and well-being of employees, hindering their ability to understand and assess the validity of system outputs and limiting their agency to exercise control over how they are represented at work.
    
    % Because AI knowledge systems thus operate on data that is subject to its own rules of transparency and privacy, access constraints, which might already enforce existing power dynamics and asymmetries within an organization, might lead to the establishment of transparency that doesn't really reflect how the system operates, nor why individuals are represented the way they are in the system. This type of transparency might allow for a type of seeing that is incomplete but might seem complete to those who see, shaping in different ways how people see \emph{into} the system and \emph{through} the system. When implemented, these forms of partial transparency can lead to interpersonal, representational and quality of service harms.

==> table-versions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SMALL FONT AND FORCED LOCATION %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
    \centering
    \caption{Questions for interrogating the intersections between ways of seeing and the three dimensions of transparency.}
    \label{tab:questions}
    \footnotesize % From Overleaf comment: Using this and H to place the table at the end of Section 3. Might not work, aesthetically, if we change much of the text - then we might need to move the table again.
    \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.15\linewidth} X X X} % >{\raggedright\arraybackslash} corrects the spacing to look nice in the first column (see p.3: https://texdoc.org/serve/tabularx/0)
      \toprule
       & System transparency & Procedural transparency & Transparency of outcomes\\
      \midrule
      \textbf{Seeing \textit{into} the system} &
        \begin{itemize}[label={}, leftmargin=*]
        \setlength\itemsep{1em} 
            \item What type of data is mined by the system and how is it used to extract knowledge?
            \item How does the system surface knowledge? E.g., what metrics does the system use to rank knowledge contributors, and how does this influence where they are surfaced or how they are presented?
        \end{itemize} &
        \begin{itemize}[label={}, leftmargin=*]
            \setlength\itemsep{1em} 
                \item In which organizational contexts is data created? Which of the organizational data is the system using? 
                \item In which organizational contexts is knowledge being surfaced?
            \end{itemize} &
        \begin{itemize}[label={}, leftmargin=*]
        \setlength\itemsep{1em} 
            \item What aspects of work are impacted by data extraction practices? How might altered work practices and outputs influence the system over time?
            \item How is the system shaping knowledge sharing practices in the organization?
        \end{itemize} \\
      \midrule
      \textbf{Seeing others individually \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What data and features does the system consider when relating someone to an area of knowledge?
          \item How reliable are surfaced associations between a given individual and knowledge?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item What actions and knowledge contributions in the organization support the associations inferred by the system? Do these reflect the way expertise is established socially in the organization?
              \item How comfortable are people with the way they are being associated with knowledge areas? E.g. are they open to be contacted about the areas they have been associated with?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How is the system shaping the way the expertise of individuals is perceived in the organization?
          \item How is the system shaping the way individuals interact with others in the organization over time?
      \end{itemize} \\
      \midrule
      \textbf{Seeing others collectively \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How does the type of data considered by the system influences who gets to be seen?
          \item What features and metrics does the system consider, and how do these influence the pieces of work and contributors that end-users see?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item Are there groups of people in the organization who contribute knowledge that is not captured by the system?
              \item What incentives in the organization drive knowledge contributions that are suitable for system extraction?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What are the impacts of disparate system performance across different demographic subgroups? How is the system shaping the exposure to different segments of people over time?
          \item How is the system shaping the establishment of objectives and measures of success in the organization?
      \end{itemize} \\
      \midrule
      \textbf{Seeing self \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What data and features does the system use to represent an individual's work? Why might algorithmic associations be incorrect and/or incomplete?
          \item How can end-users know and control how they're represented by the system?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item How well does the surfaced system representation match individuals’ self-perception?
              \item How can end-users know and control how they're seen by others through the system? Do people in the organization have different levels of visibility into and/or control of how they're seen?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How are individuals adapting their behavior towards knowledge creation and sharing to bridge their self-perception and the system representation?
          \item Can individuals tell how changes in their behavior influence system behavior over time?
      \end{itemize} \\
      \bottomrule
    \end{tabularx}
\end{table}
% [label={}] is from https://tex.stackexchange.com/questions/50269/itemize-without-bullets
% [leftmargin=*] is from https://tex.stackexchange.com/questions/91124/itemize-removing-natural-indent
% \setlength\itemsep{1em} is from https://tex.stackexchange.com/questions/12373/how-to-change-the-space-between-the-itemize-items-in-latex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% REGULAR FONT, LATEX DECIDES LOCATION %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
    \centering
    \caption{Questions for interrogating the intersections between ways of seeing and the three dimensions of transparency.}
    \label{tab:questions}
    %\footnotesize
    \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.15\linewidth} X X X} % >{\raggedright\arraybackslash} corrects the spacing to look nice in the first column (see p.3: https://texdoc.org/serve/tabularx/0)
      \toprule
       & System transparency & Procedural transparency & Transparency of outcomes\\
      \midrule
      \textbf{Seeing \textit{into} the system} &
        \begin{itemize}[label={}, leftmargin=*]
        \setlength\itemsep{1em} 
            \item What type of data is mined by the system and how is it used to extract knowledge?
            \item How does the system surface knowledge? E.g., what metrics does the system use to rank knowledge contributors, and how does this influence where they are surfaced or how they are presented?
        \end{itemize} &
        \begin{itemize}[label={}, leftmargin=*]
            \setlength\itemsep{1em} 
                \item In which organizational contexts is data created? Which of the organizational data is the system using? 
                \item In which organizational contexts is knowledge being surfaced?
            \end{itemize} &
        \begin{itemize}[label={}, leftmargin=*]
        \setlength\itemsep{1em} 
            \item What aspects of work are impacted by data extraction practices? How might altered work practices and outputs influence the system over time?
            \item How is the system shaping knowledge sharing practices in the organization?
        \end{itemize} \\
      \midrule
      \textbf{Seeing others individually \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What data and features does the system consider when relating someone to an area of knowledge?
          \item How reliable are surfaced associations between a given individual and knowledge?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item What actions and knowledge contributions in the organization support the associations inferred by the system? Do these reflect the way expertise is established socially in the organization?
              \item How comfortable are people with the way they are being associated with knowledge areas? E.g. are they open to be contacted about the areas they have been associated with?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How is the system shaping the way the expertise of individuals is perceived in the organization?
          \item How is the system shaping the way individuals interact with others in the organization over time?
      \end{itemize} \\
      \midrule
      \textbf{Seeing others collectively \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How does the type of data considered by the system influences who gets to be seen?
          \item What features and metrics does the system consider, and how do these influence the pieces of work and contributors that end-users see?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item Are there groups of people in the organization who contribute knowledge that is not captured by the system?
              \item What incentives in the organization drive knowledge contributions that are suitable for system extraction?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What are the impacts of disparate system performance across different demographic subgroups? How is the system shaping the exposure to different segments of people over time?
          \item How is the system shaping the establishment of objectives and measures of success in the organization?
      \end{itemize} \\
      \midrule
      \textbf{Seeing self \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What data and features does the system use to represent an individual's work? Why might algorithmic associations be incorrect and/or incomplete?
          \item How can end-users know and control how they're represented by the system?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item How well does the surfaced system representation match individuals’ self-perception?
              \item How can end-users know and control how they're seen by others through the system? Do people in the organization have different levels of visibility into and/or control of how they're seen?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How are individuals adapting their behavior towards knowledge creation and sharing to bridge their self-perception and the system representation?
          \item Can individuals tell how changes in their behavior influence system behavior over time?
      \end{itemize} \\
      \bottomrule
    \end{tabularx}
\end{table}
% [label={}] is from https://tex.stackexchange.com/questions/50269/itemize-without-bullets
% [leftmargin=*] is from https://tex.stackexchange.com/questions/91124/itemize-removing-natural-indent
% \setlength\itemsep{1em} is from https://tex.stackexchange.com/questions/12373/how-to-change-the-space-between-the-itemize-items-in-latex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SEPARATE TABLES (FORCED LOCATION) %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
    \centering
    \caption{Questions for interrogating the intersections between ways of seeing and the three dimensions of transparency.}
    \label{tab:questions}
    %\footnotesize
    \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.15\linewidth} X X X} % >{\raggedright\arraybackslash} corrects the spacing to look nice in the first column (see p.3: https://texdoc.org/serve/tabularx/0)
      \toprule
       & System transparency & Procedural transparency & Transparency of outcomes\\
      \midrule
      \textbf{Seeing \textit{into} the system} &
        \begin{itemize}[label={}, leftmargin=*]
        \setlength\itemsep{1em} 
            \item What type of data is mined by the system and how is it used to extract knowledge?
            \item How does the system surface knowledge? E.g., what metrics does the system use to rank knowledge contributors, and how does this influence where they are surfaced or how they are presented?
        \end{itemize} &
        \begin{itemize}[label={}, leftmargin=*]
            \setlength\itemsep{1em} 
                \item In which organizational contexts is data created? Which of the organizational data is the system using? 
                \item In which organizational contexts is knowledge being surfaced?
            \end{itemize} &
        \begin{itemize}[label={}, leftmargin=*]
        \setlength\itemsep{1em} 
            \item What aspects of work are impacted by data extraction practices? How might altered work practices and outputs influence the system over time?
            \item How is the system shaping knowledge sharing practices in the organization?
        \end{itemize} \\
      \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[H]
    \centering
    \caption{Questions for interrogating the intersections between ways of seeing and the three dimensions of transparency.}
    \label{tab:questions}
    %\footnotesize
    \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.15\linewidth} X X X} % >{\raggedright\arraybackslash} corrects the spacing to look nice in the first column (see p.3: https://texdoc.org/serve/tabularx/0)
      \toprule
       & System transparency & Procedural transparency & Transparency of outcomes\\
      \midrule
      \textbf{Seeing others individually \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What data and features does the system consider when relating someone to an area of knowledge?
          \item How reliable are surfaced associations between a given individual and knowledge?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item What actions and knowledge contributions in the organization support the associations inferred by the system? Do these reflect the way expertise is established socially in the organization?
              \item How comfortable are people with the way they are being associated with knowledge areas? E.g. are they open to be contacted about the areas they have been associated with?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How is the system shaping the way the expertise of individuals is perceived in the organization?
          \item How is the system shaping the way individuals interact with others in the organization over time?
      \end{itemize} \\
      \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[H]
    \centering
    \caption{Questions for interrogating the intersections between ways of seeing and the three dimensions of transparency.}
    \label{tab:questions}
    %\footnotesize
    \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.15\linewidth} X X X} % >{\raggedright\arraybackslash} corrects the spacing to look nice in the first column (see p.3: https://texdoc.org/serve/tabularx/0)
      \toprule
       & System transparency & Procedural transparency & Transparency of outcomes\\
      \midrule
      \textbf{Seeing others collectively \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How does the type of data considered by the system influences who gets to be seen?
          \item What features and metrics does the system consider, and how do these influence the pieces of work and contributors that end-users see?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item Are there groups of people in the organization who contribute knowledge that is not captured by the system?
              \item What incentives in the organization drive knowledge contributions that are suitable for system extraction?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What are the impacts of disparate system performance across different demographic subgroups? How is the system shaping the exposure to different segments of people over time?
          \item How is the system shaping the establishment of objectives and measures of success in the organization?
      \end{itemize} \\
      \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[H]
    \centering
    \caption{Questions for interrogating the intersections between ways of seeing and the three dimensions of transparency.}
    \label{tab:questions}
    %\footnotesize
    \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.15\linewidth} X X X} % >{\raggedright\arraybackslash} corrects the spacing to look nice in the first column (see p.3: https://texdoc.org/serve/tabularx/0)
      \toprule
       & System transparency & Procedural transparency & Transparency of outcomes\\
      \midrule
      \textbf{Seeing self \textit{through} the system} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item What data and features does the system use to represent an individual's work? Why might algorithmic associations be incorrect and/or incomplete?
          \item How can end-users know and control how they're represented by the system?
      \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
          \setlength\itemsep{1em} 
              \item How well does the surfaced system representation match individuals’ self-perception?
              \item How can end-users know and control how they're seen by others through the system? Do people in the organization have different levels of visibility into and/or control of how they're seen?
          \end{itemize} &
      \begin{itemize}[label={}, leftmargin=*]
      \setlength\itemsep{1em} 
          \item How are individuals adapting their behavior towards knowledge creation and sharing to bridge their self-perception and the system representation?
          \item Can individuals tell how changes in their behavior influence system behavior over time?
      \end{itemize} \\
      \bottomrule
    \end{tabularx}
\end{table}
% [label={}] is from https://tex.stackexchange.com/questions/50269/itemize-without-bullets
% [leftmargin=*] is from https://tex.stackexchange.com/questions/91124/itemize-removing-natural-indent
% \setlength\itemsep{1em} is from https://tex.stackexchange.com/questions/12373/how-to-change-the-space-between-the-itemize-items-in-latex
